Weighted Essentially Non-Oscillatory stochastic Galerkin approximation for hyperbolic conservation laws

In this paper we extensively study the stochastic Galerkin scheme for uncertain systems of conservation laws, which appears to produce oscillations already for a simple example of the linear advection equation with Riemann initial data. Therefore, we introduce a modified scheme that we call the weighted essentially non-oscillatory (WENO) stochastic Galerkin scheme, which is constructed to prevent the propagation of Gibbs phenomenon into the stochastic domain by applying a slope limiter in the stochasticity. In order to achieve a high order method, we use a spatial WENO reconstruction and also compare the results to a scheme that uses WENO reconstruction in both the physical and the stochastic domain. We evaluate these methods by presenting various numerical test cases where we observe the reduction of the total variation compared to classical stochastic Galerkin.

==> Sections/model_backup_v.tex <==
\section{Modeling Uncertainties}\label{sec:model}

We consider stochastic conservation laws of the form
%
\begin{equation}\label{eq:spde}
 \pd{\timevar} \solution(\timevar,\x,\uncertainty) + \pd{\x} \flux\bigl(\solution(\timevar,\x,\uncertainty),\xi\bigr) = 0,\quad \quad \text{for} \ \ \x\in\PD,\, t>0,\, \uncertainty\in\SD\,,
\end{equation}
%
with physical domain $\PD \subset \RR$, stochastic domain $\SD \subset \RR$ and the following initial conditions
%
\begin{equation*}
 \solution(0,\x,\uncertainty) = \solution^{(0)}(\x,\uncertainty), \quad \quad \text{for} \ \ \x\in\PD,\, \xi\in\SD\,.
\end{equation*}
%
Depending on $\PD$, additional boundary conditions have to be given.
%
The solution $\solution\in\RR^\dimension$ is depending on a one-dimensional random variable $\uncertainty$ with probability space $(\sampleSpace,\sigmaAlgebra,\probabilityMeasure)$.
We denote the random space of this uncertainty by $\randomSpace := \uncertainty(\sampleSpace)$ and its probability density function by $\xiPDF(\uncertainty) : \randomSpace \rightarrow \R_+$.

\subsection{Stochastic Galerkin}
We seek for an approximate solution by a finite-term generalized Polynomial Chaos (gPC) expansion (see e.g.\ \cite{Gottlieb2008}),
%
\begin{equation}\label{gPCApprox}
\solution(\timevar,\x,\uncertainty) \approx  \sum\limits_{\SGsumIndex=0}^{\SGtruncorder} \solution_\SGsumIndex(\timevar,\x) \, \xiBasisPoly{\SGsumIndex}(\uncertainty) \,,
\end{equation}
%
where the polynomials $\xiBasisPoly{\SGsumIndex}$ (of degree $\SGsumIndex$) are supposed to satisfy the orthogonality relation
%
\begin{equation}\label{eq:orthogonality}
\int\limits_{\randomSpace} \xiBasisPoly{\SGsumIndex}(\uncertainty) \, \xiBasisPoly{\SGeqIndex}(\uncertainty) \, \xiPDF(\uncertainty) \dint{\uncertainty} = \delta_{\SGsumIndex\SGeqIndex}, \quad \quad \forall \SGsumIndex,\SGeqIndex \in \{0, \dots, \SGtruncorder\}.
\end{equation}
Inserting \eqref{gPCApprox} into \eqref{eq:spde} and applying a Galerkin projection (in the stochastic space) leads to the stochastic Galerkin system
$$ \pd{t} \solution_\SGeqIndex +  \pd{\x} \intRS \flux\!\left(\SGapproach\right) \!\xiBasisPoly{\SGeqIndex}\xiPDFdxi = 0, \qquad \SGeqIndex = 0,\ldots,\SGtruncorder.$$


\subsection{\ME{} Ansatz}
For discontinuous solutions, the gPC approach may converge slowly or even fail to converge, cf. \cite{Wan2005, Poette2009}.  As presented in \cite{Wan2006,Meyer2018}, we therefore apply the \ME{} approach, where $\randomSpace$ is divided into disjoint elements with local gPC approximation of  \eqref{eq:spde}.

We assume that $\randomSpace=(\uncertainty_L,\uncertainty_R)$ and define a decomposition of $\randomSpace$ as $ \uncertainty_L= d_1 < d_2 < \ldots < d_{\MEElements+1}= \uncertainty_R$ with \ME{}s $\randomElement{\MEIndex} = (d_\MEIndex, d_{\MEIndex+1})$, for $ \MEIndex= 1,\ldots, \MEElements$.  Moreover, we  introduce an indicator variable $\chi_{\MEIndex}: \Omega \to  \{0,1\}$ on every random element
\begin{equation}\label{def:indicator}
\indicatorVar{\MEIndex}{\uncertainty(\omega)} :=
\begin{cases}
1, &\text{if } \uncertainty(\omega) \in \randomElement{\MEIndex}, \\
0, &\text{else, }
\end{cases}
\end{equation}
for $\MEIndex=1,\ldots,\MEElements $ and $\omega\in\sampleSpace$. 
%Using the indicator variable allows us to derive a disjoint partition of the sample space $\sampleSpace$ via
%\begin{equation*}
%\sampleSpace  = \bigcup \limits_{\MEIndex=1}^\MEElements \inverseIndicator{\MEIndex}{1}.
%\end{equation*}
%Hence, we can define a new local random variable $\localuncertainty{\MEIndex}: \inverseIndicator{\MEIndex}{1} \to \randomElement{\MEIndex}$ on the local probability space $(\inverseIndicator{\MEIndex}{1},\sigmaAlgebra\cap \inverseIndicator{k}{1},\probabilityMeasure(\cdot | \indicatorVar{\MEIndex}{\uncertainty} =1))$. Using Bayes' rule we compute the following local probability 
%density functions 
%\begin{equation}\label{def:CondDensity}
%\locxiPDF{\MEIndex}:=\locxiPDF{\MEIndex}(\localuncertainty{\MEIndex}|\indicatorVar{\MEIndex}{\uncertainty}=1) = %\frac{\xiPDF(\localuncertainty{\MEIndex})}{\probabilityMeasure(\indicatorVar{\MEIndex}{\uncertainty}=1)},\qquad \MEIndex=1,\ldots,\MEElements.
%\end{equation}
%\begin{remark}
%	For a uniform distribution of the uncertainty, we have $\locxiPDF{\MEIndex}=\frac{1}{d_{\MEIndex+1}-d_\MEIndex}$.
%\end{remark}
If we let $\{\localxiBasisPoly{\SGsumIndex}{\MEIndex} (\localuncertainty{\MEIndex})\}_{\SGsumIndex=0}^\infty$ be  orthonormal polynomials with respect to a conditional probability density function on the \ME{} $\randomElement{\MEIndex}$, cf. \cite{Meyer2018}, 
%we may consider the local gPC approximation in an element $\randomElement{\MEIndex}$,
%\begin{equation}
%\solution_{\MEIndex}(t,x,\localuncertainty{\MEIndex}) \approx
%\sum_{\SGsumIndex=0}^{\SGtruncorder} \solution_{\SGsumIndex, \MEIndex}(\timevar,\x) \localxiBasisPoly{\SGsumIndex}{\MEIndex} (\localuncertainty{\MEIndex}),
%\end{equation}
%for all $\MEIndex =1,\ldots,\MEElements$.
the global approximation \eqref{gPCApprox} can be written as
\begin{equation}\label{def:globalSG}
\solution(t,x,\uncertainty) = \sum_{\MEIndex=1}^{\MEElements}  \solution_\MEIndex(t,x,\uncertainty) \indicatorVar{\MEIndex}{\uncertainty} \approx \sum_{\MEIndex=1}^{\MEElements}  \sum_{\SGsumIndex=0}^{\SGtruncorder}  \solution_{\SGsumIndex, \MEIndex}(\timevar,\x) \localxiBasisPoly{\SGsumIndex}{\MEIndex}(\uncertainty) \indicatorVar{\MEIndex}{\uncertainty}.
\end{equation}
As $\MEElements,\SGtruncorder\to\infty$, the local approximation converges to the global solution in $\Lp{2}(\sampleSpace)$, cf \cite{Alpert1993}.

The calculation of the expected value and the variance can be found in \cite{Meyer2018}.

\begin{remark}\label{rem:disjointME}
	The stochastic Galerkin scheme can be applied to every \ME{} separately, due to the disjoint decomposition of the random space.
\end{remark}

\subsection{Propagation of the Gibbs phenomenon}\label{sec:LAex}
\todo{some blabla about gibbs phenomenon for hyperbolic equations and transition from space to probability}
As introductory example, we consider the one-dimensional hyperbolic problem
%
\begin{equation}\label{stochasticWaveEquation}
 u_t + a(\xi) \, u_x = 0
\end{equation}
%
with $x\in(0,\infty)$ and uncertain wave speed
%
\begin{equation}\label{stochasticWaveSpeed}
 a(\xi) = 1.5 + 0.5\, \xi\,,
\end{equation}
%
where $\xi \sim U(-1,1)$, i.e., $\xi$ is uniformly distributed in $[-1,1]$. Hence, the density function is given by $\xiPDF=0.5$ and the basis functions $\xiBasisPoly{k}$ by the Legendre polynomials orthonormalized wrt. \eqref{eq:orthogonality}.
%
Further, we use non-smooth initial data
%
\begin{equation}\label{sweInitialConditions}
 u(0,\x,\xi) = u^{(0)}(x) = \begin{cases}
           1 & \text{for } 0 \le x \le 0.5\,,\\
	   0 & \text{for } 0.5 < x\,,
          \end{cases}
\end{equation}
%
and constant boundary data
%
\begin{equation}\label{sweBoundaryConditions}
 u(t,0,\xi) = 1 \,.
\end{equation}

We approximate the solution by the Polynomial Chaos (gPC) expansion \eqref{gPCApprox}
%
\begin{equation}\label{LAgPC}
 u(t,x,\xi) \approx v(t,x,\xi) = \sum\limits_{\SGsumIndex=0}^{\SGtruncorder} u_\SGsumIndex(\timevar,\x) \, \xiBasisPoly{\SGsumIndex}(\uncertainty).
\end{equation}
%
Inserting \eqref{LAgPC} in \eqref{stochasticWaveEquation} and applying a Galerkin projection (in the stochastic space) leads to
%
\begin{equation*}
 \pd{t} u_l(t,x) + \sum\limits_{k=0}^{\SGtruncorder} a_{l,k} \pd{x} u_k(t,x) = 0, \quad \quad \text{for} \ \ l = 0, \dots, \SGtruncorder
\end{equation*}
%
with
%
\begin{equation*}
 a_{l,k} = \int\limits_{-1}^{1} a(\xi) \xiBasisPoly{l}(\xi) \xiBasisPoly{k}(\xi) \xiPDF(\xi) \dint{\xi} \,.
\end{equation*}

Collecting all $u_l$ into a vector $V = (u_0, \dots, u_\SGtruncorder)^T$ and the $a_{l,k}$ into a matrix $A$ yields the system
%
\begin{equation}\label{sweProjection}
 \pd{t} V(t,x) + A \pd{x} V(t,x) = 0\,.
\end{equation}
%
Note that this system is hyperbolic because $A = A^T$.

The Galerkin projection of the initial conditions \eqref{sweInitialConditions} gives
%
\begin{equation*}
u_l(0,x) = \int\limits_{-1}^{1} u^{(0)}(x,\xi) \xiBasisPoly{l}(\xi) \xiPDF(\xi) \dint{\xi} = u^{(0)}(x) \int\limits_{-1}^{1} \!\xiBasisPoly{l}(\xi) \xiPDF(\xi) \dint{\xi}, \quad \quad \text{for} \ \ l = 0, \dots, \SGtruncorder\,.
\end{equation*}
%
and therewith
%
\begin{equation*}
 V(0,x) = \begin{pmatrix}
           u^{(0)}(x)\\ 0\\ \vdots\\ 0
          \end{pmatrix}\,.
\end{equation*}

For the boundary conditions \eqref{sweBoundaryConditions} the Galerkin projection leads to
%
\begin{equation*}
 u_l(t,0,\xi) = \int\limits_{-1}^{1} u(t,0,\xi) \xiBasisPoly{l}(\xi) \xiPDF(\xi) \dint{\xi} = \int\limits_{-1}^{1} \xiBasisPoly{l}(\xi) \xiPDF(\xi) \dint{\xi}, \quad \quad \text{for} \ \ l = 0, \dots, \SGtruncorder
\end{equation*}
%
and therewith
%
\begin{equation*}
 V(t,0) = \begin{pmatrix}
           1\\ 0\\ \vdots\\ 0
          \end{pmatrix}\,.
\end{equation*}

Since \eqref{sweProjection} is a linear hyperbolic system, it can be decoupled into $\SGtruncorder$ scalar transport equations and the analytic solution can be explicitly given. For this purpose, we introduce a new variable $W := T^{-1} V$, where $T$ is the matrix of eigenvectors of $A$ (columnwise). With $\lambda_j$ being the corresponding (real) eigenvalues, the components of $W$ satisfy
%
\begin{equation*}
 \pd{t} W_j + \lambda_j \pd{x} W_j = 0, \quad \quad \text{for} \ \ j = 0, \dots, \SGtruncorder
\end{equation*}
%
and the solution of the Galerkin system is given by
%
\begin{equation*}
 W_j(t,x) = \begin{cases}
             \big( T^{-1} V(x-\lambda_j t,0) \big)_j\quad & \text{for } x-\lambda_j t \ge 0\,,\\
	     \big( T^{-1} V(0,t-\frac{x}{\lambda_j}) \big)_j & \text{for } x-\lambda_j t \le 0\,.
            \end{cases}
\end{equation*}


For the following considerations, we use $\SGtruncorder=2$. From \eqref{eq:orthogonality} we deduce the Legendre polynomials
%
\begin{equation*}
 \xiBasisPoly{0}(\xi) = 1\,, \quad \xiBasisPoly{1}(\xi) = \sqrt{3} \xi\,, \quad \xiBasisPoly{2}(\xi) = \tfrac{\sqrt{5}}{2} (3\xi^2-1)\,,
\end{equation*}
%
and further
%
\begin{equation*}
 A = \begin{pmatrix}
      \frac32 & \frac{\sqrt{3}}6 & 0\\
      \frac{\sqrt{3}}6 & \frac32 & \frac{\sqrt{15}}{15}\\
      0 & \frac{\sqrt{15}}{15} & \frac32
     \end{pmatrix}\,.
\end{equation*}
%
The eigenvalues of $A$ are $\tfrac32 - \tfrac{\sqrt{15}}{10}$, $\tfrac32$ and $\tfrac32 + \tfrac{\sqrt{15}}{10}$. Interestingly, the corresponding $\xi$s (via \eqref{stochasticWaveSpeed}) are the zeros of the third order Legendre polynomial and our finite-term expansion \eqref{LAgPC} is exact for those $\xi$s. Accordingly, the gPC Galerkin approximation $v(x,t,\xi)$ (given by \eqref{LAgPC}) here equals the quadratic interpolating polynomial in the stochastic space with sampling points $\xi \in \{-\sqrt{\tfrac{3}{5}}, 0, \sqrt{\tfrac{3}{5}}\}$.
%As mentioned above, the gPC Galerkin approximation $v(x,t,\xi)$ given by \eqref{gPCApprox} is exact for $\xi \in \{\tfrac32 - \tfrac{\sqrt{15}}{10}, \tfrac32, \tfrac32 + \tfrac{\sqrt{15}}{10}\}$ and therefore coincides with the corresponding quadratic interpolating polynomial.
Now, the problem is that the discontinuity with respect to $x$ in the initial conditions \eqref{sweInitialConditions} carries over to the stochastic domain. This leads to overshoots (Gibbs phenomena) in the gPC Galerkin approximation as illustrated in Figure~\ref{fig:gPCApprox} for $t=0.5$ and a choice of $\xi$s inside and outside of the convex hull of the sampling points.

\input{Sections/figureGPCx}

Note that this effect does not result from the fact that we made a global ansatz in the stochastic space but from the lack of regularity (see below). Moreover, if we want to refine the grid in the stochastic space close to the discontinuity, we are faced with the problem that the position of the jump in the stochastic space depends on $x$ and $t$ as illustrated in Figure~\ref{fig:discStochasticSpace}. A short computation yields $$\xi_{\text{jump}} = \frac{2x-1}{t} - 3$$ so that at $t=0.5$ the position of the discontinuity in the stochastic space takes all values in $[-1,1]$ for $x \in [1,1.5]$.

\input{Sections/figureGPCxi}

Now, as noted above, we demonstrate that a grid refinement in the sense of a \ME{} approach does only marginally improve the so-found approximation. For this, we briefly consider the case where the stochastic domain is equally partitioned into three intervals and we apply the gPC Galerkin approach in each of them. With respect to the stochastic domain, this results in a discontinuous Galerkin approximation of the entire solution and the approximation in each interval can be independently computed analogously to the procedure described above.
Now, we look at the so-found approximations for some $\xi_j \in [-\tfrac13, \tfrac13]$ and compare them with the global gPC Galerkin approximations from above at $3\xi_j \in [-1,1]$. Certainly, we are looking at approximations to different solutions this way, but we are interested in another property of the solution manifold: As one can easily see from the plots in Figure~\ref{fig:gPCRefined}, the width of the overshoots in the compared approximations reduced but the height remained, which is a well-known issue for Gibbs phenomena. Thus, solely the refinement of the grid in the stochastic space cannot reduce the overshoots in the solution manifold.

\input{Sections/figureGPCrefined}

\subsection{Slope Limiter} \label{sec:slopeLimiter}
We now consider a slope limiter within the stochastic space to reduce the oscillations described in the previous subsection. We present the minimod limiter \cite{Cockburn1989a,Cockburn1991}, given by the following troubled cell indicator for the $j$th \ME{} $\randomElement{\MEIndex}$
\begin{equation}\label{eq:TCminmod}
TC_j(\solution) = \begin{cases}
1, & \solution_{1,j} \neq \text{m}\big(\solution_{1,j},\, \solution_{0,j+1}-\solution_{0,j}, \, \solution_{0,j}-\solution_{0,j-1}\big)\\
0, & \text{otherwise},
\end{cases}
\end{equation}
where $\text{m}(\cdot,\cdot,\cdot)$ is the minmod function and $\solution_{k,j}$, $k=0,1$, are the $k$th coefficients of the local gPC representations of the solution $\solution$ in the $j$th \ME{} as in \eqref{def:globalSG}. At the boundary, we repeat the entries of the first (last) \ME{}. Finally, we replace each coefficient of $\solution\big|_{D_j}$ for $j=1,\ldots,\MEElements$ by
\begin{equation}\label{eq:slopeLimiter}
\hat \solution\big|_{D_j} =\begin{pmatrix}
\hat \solution_{0,j}\\ \hat \solution_{1,j}\\ \vdots \\ \hat \solution_{\SGtruncorder,j}
\end{pmatrix} = \begin{cases}
\begin{pmatrix}
(\solution_{0,j})^T\\[0.2cm]
 \text{m}\big(\solution_{1,j},\, \solution_{0,j+1}-\solution_{0,j}, \, \solution_{0,j}-\solution_{0,j-1}\big)\\[0.2cm]
 (0,\ldots,0)^T\\
 \vdots\\
 (0,\ldots,0)^T
\end{pmatrix}, & \text{if } TC_j(\solution) = 1 \\[1.5cm]
\quad \solution\big|_{D_j}\,, & \text{otherwise}.
\end{cases}\end{equation}
Hence, we assume that the oscillations in the solution vector are mainly generated in the part with linear uncertainty \cite{Shu1987}.

\begin{remark}
	The troubled cell indicator \eqref{eq:TCminmod} is defined for an expansion of $\solution$ in monomials. If the SG basis polynomials $\xiBasisPoly{0}$ and $\xiBasisPoly{1}$ are given by other functions we need to adapt this definition. For example in the case of Legendre polynomials we have to multiply $\solution_{1,j}$ by $\sqrt{3}$ before inserting it into the minmod function.
\end{remark}

If $\SGtruncorder\geq2$, we only apply the slope limiter if 
$|\solution_{1,j}| \geq M | \randomElement{\MEIndex} |^2$
in addition to $TC_j(\solution) = 1$ to achieve the TVBM property. The constant $M$ is chosen according to \cite{quarteroni2006advanced}
$$M = \text{sup}\Big\{|\partial_x^2\solution_{t=0}| ~\Big|~ \x\in\Domain,\,\partial_x\solution_{t=0}=0\Big\}.$$

%In our numerical studies we will mainly	 use a WENO limiter combined with the minmod troubled cell indicator $TC_j(\solution)$ described in \eqref{eq:TCminmod}. The solution in the troubled \ME{}s is then replaced by its WENO reconstruction in the stochastic space, ie. in the \ME{}.

The slope limited gPC Galerkin approximation can now be applied to the linear advection example from Section \ref{sec:LAex}. \figref{fig:gPClimiter}  compares the gPC approximation in 3 \ME{}s with its slope limited version (dashed), which reduced the overshoots tremendously. The application of the minmod slope limiter in the stochastic space \eqref{eq:slopeLimiter} has been sufficient to prevent Gibbs phenomenon.

\input{Images/figureGPClimiter}

In \figref{fig:gPClimiter_refined} we kept refining the number of \ME{}s to 10, where Gibbs phenomenon still causes overshoots of the same height as before. The slope limiter (dashed) completely eliminated these oscillations.

\input{Images/figureGPClimiter_refined}

